BERT for Coreference Resolution: Baselines and Analysis

We apply BERT to coreference resolution, achieving strong improvements on the OntoNotes (+3.9 F1) and GAP (+11.5 F1) benchmarks. A qualitative analysis of model predictions indicates that, compared to ELMo and BERT-base, BERT-large is particularly better at distinguishing between related but distinct entities (e.g., President and CEO). However, there is still room for improvement in modeling document-level context, conversations, and mention paraphrasing. Our code and models are publicly available.

==> conclusion.tex <==
\section{Conclusion}
We present state of the art results for coreference resolution on GAP and OntoNotes benchmarks. While the gains on paragraph-level coreference (GAP) are substantial, the improvement on document-level coreference (OntoNotes) is more modest. We hypothesize that even with BERT's large-scale paragraph level pretraining, current models are unable to leverage information from longer contexts. Overall, OntoNotes, on account of being a document-level task, is still a difficult benchmark for coreference resolution.

